Making Reasoning Matter: Measuring and Improving Faithfulness of Chain-of-Thought Reasoning

Large language models (LLMs) have been shown to perform better when asked to reason step-by-step before answering a question. However, it is unclear to what degree the model's final answer is faithful to the stated reasoning steps. In this paper, we perform a causal mediation analysis on twelve LLMs to examine how intermediate reasoning steps generated by the LLM influence the final outcome and find that LLMs do not reliably use their intermediate reasoning steps when generating an answer. To address this issue, we introduce FRODO, a framework to tailor small-sized LMs to generate correct reasoning steps and robustly reason over these steps. FRODO consists of an inference module that learns to generate correct reasoning steps using an implicit causal reward function and a reasoning module that learns to faithfully reason over these intermediate inferences using a counterfactual and causal preference objective. Our experiments show that FRODO significantly outperforms four competitive baselines. Furthermore, FRODO improves the robustness and generalization ability of the reasoning LM, yielding higher performance on out-of-distribution test sets. Finally, we find that FRODO's rationales are more faithful to its final answer predictions than standard supervised fine-tuning.

==> 00_instruction.tex <==

\section{Submission of conference papers to ICLR 2024}

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NeurIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2024 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2024_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2024_conference.sty+ and \verb+iclr2024_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2024_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 9 pages for the main text of the initial submission, with unlimited additional pages for citations. 

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.

\subsubsection*{Author Contributions}
If you'd like to, you may include  a section for author contributions as is done
in many journals. This is optional and at the discretion of the authors.

\subsubsection*{Acknowledgments}
Use unnumbered third level headings for the acknowledgments. All
acknowledgments, including those to funding agencies, go at the end of the paper.


==> 02_preliminaries_copy.tex <==
\section{Reasoning Chain as a Mediator}\label{sec:reasoning_causal}

\textbf{Problem Formulation.} Reasoning is often a process that involves composing multiple inference steps to reach a conclusion or make a decision. We informally conceptualize each reasoning task as requiring a model $f$: $X$ → $Y$ to map an input $x \in X$ to an output $y \in Y$ by making correct or plausible inference steps $R$. 

%In this paper, we view \textit{natural language reasoning} (NLR) as an autoregressive generation task where, given input context $x$, a model needs to generate $y$, such that $y$ satisfies the constraints of the task. Usually, to generate correct or plausible $y$, the model must make the correct inference $z$ as intermediate steps. We consider the prior knowledge as the context representation $x$, encoded by the pre-trained LM $\theta$. 

%We decompose NLR tasks as follows: 
%\begin{equation}
%    p(y|x) = p(y|x,z) p(z|x).
%\end{equation}
%In practice, one can compute each conditional using an LM that includes its conditioning variables as a part of its input.  
\textbf{Causal Interpretation.} The causal graph is a probabilistic graphical model used to describe how variables interact, expressed by a directed acyclic graph consisting of the sets of nodes ($N$) denoting the variables and the edges ($E$) between the nodes denoting the causality \citep{Pearl1998GraphsCA}. As shown in Fig. \ref{fig:causal_graph}(a), if $Y$ is a descendent of $X$, then $X$ is a potential cause of $Y$, and $Y$ is the effect.

\textbf{Causal mediation analysis.} It is a method of causal inference which studies the change in a dependent variable following an intervention or treatment of an independent variable \citep{Pearl2001DirectAI}. Causal mediation analysis aims to decompose the total effect of the independent variable ($X$) on the dependent variable ($Y$) into two components: the direct effect and the indirect effect \citep{Pearl2001DirectAI}. In this work, we view the reasoning process as a causal graph, framing the input (reasoning problem) $X$ and the output $Y$ as random variables and the reasoning steps as mediator variable $R$.  We use mediation analysis to interpret the role of reasoning steps as mediators between model inputs and model outputs. Please note that there are two mediator variables, model parameters $M$ and reasoning steps $R$ (see Fig. \ref{fig:causal_graph}(b)). However, in this work, we are interested in understanding the indirect effect of $R$ on the output $Y$; hence, we assume model parameters $M$ to be fixed. 
Let $X_0$ denote the initial reasoning problem, $R_0$ as the reasoning chain given $X_0$ and $Y_{00}$ denote the potential outcome if the treatment variable and mediator variable are $X_0$ and $R_0$, respectively. Whereas $Y_{01}$ denotes the possible outcome when treatment is set to $X_0$ and $R_1$ is the reasoning chain for an intervened reasoning problem (see Fig.\ref{fig:causal_graph}(d)). 

\begin{figure}[t]
    \centering   
    \includegraphics[scale=1,height=5.5 cm, width=0.35\paperwidth]{figure/CSM.png}
    \caption{Causal graph for natural language reasoning, where we model $P(Y| do(x))$. $X_0$ = original reasoning problem, $X_1$ = intervened reasoning problem, $R_0$ = reasoning steps for $X_0$ reasoning problem, $R_1$ = reasoning steps for $X_1$, $Y$ = output, and $M$ = model parameters}
    \vspace*{-5mm}
    \label{fig:causal_graph}
\end{figure} 
%Let Y(ω) denote some post-treatment outcome for individual ω. Let Z(ω) be a post-treatment variable that will denote the intermediate variable. Let Ya(ω) and Za(ω) denote respectively the counterfactual values (or potential outcomes) of Y and Z for individual ω if treatment A were set, possibly contrary to fact, to the value a. 

% The \textit{direct effect} represents the impact of the independent variable on the dependent variable that occurs without the influence of intermediate variables or mediators ($Z$) (see Fig. \ref{fig:causal_graph}(a)). The \textit{indirect effect} represents the impact of the independent variable on the dependent variable that occurs through one or more intermediary variables or mediators.

\textit{Direct Effect} (DE) measures how much an intervention $X$ changes an outcome variable $Y$ directly, without passing through a hypothesized mediator $R$. Based on Fig \ref{fig:causal_graph}(c), we define the direct effect of $X$=$X_0$ on $Y$ as $DE = P(Y|X_0, R_0) - P(Y|X_1,R_0)$ which can be seen as the comparisons between two potential outcomes of $X$ given two different treatments, i.e., $X$ = $X_0$ and $X_1$. It is computed by applying the intervention $X$ but holding $R$ fixed to its original value ($R_0$). 

\textit{Indirect Effect} measures how much the intervention $X$ changes $Y$ indirectly through $R$. We define the indirect effect as $IE = P(Y|X_0,R_0) - P(Y|X_0,R_1)$. It is computed by setting $R$ to its value under the intervention $X$ while keeping everything else to its original value.

More concretely, a high direct effect means that $X$ has higher causality on $Y$, i.e., the model puts more emphasis on the reasoning problem than the reasoning steps. In contrast, a high indirect effect means the model puts more emphasis on the reasoning steps than the problem input.
\begin{table}[t!]
\centering
\scalebox{0.7}{
\begin{tabular}{@{}c@{~~}l@{~~}}
\toprule
{\bf Variables } & {\bf Example}\\\midrule
%\rowcolor{gray!25}
%\textbf{Full training data} &  &\\
 
%Y_00 = model generated output when conditioned on X_0 and R_0 & \\
%y_01 = model generated output when conditioned on x_0 and r_1
%y_10 = model generated output when conditioned on x_1 and r_0
%y_11 = model generated output when conditioned on x_1 and r_1`
$X_0$ & \textit{Is Poseidon similar to the god Vulcan?} \\ 
$X_1$ & \textit{Is Poseidon similar to the god Neptune?} \\ 
$R_0$ & \textit{Poseidon is a god from Greek mythology, known} \\ 
& \textit{as the god of the sea, earthquakes, and horses.} \\
& \textit{Vulcan is a god from Roman mythology, known} \\ 
& \textit{as the god of fire, metalworking, and the forge.} \\
& \textit{Although both are gods, they represent different} \\
& \textit{elements and aspects, and come from} \\
& \textit{different mythologies.} \\
$R_1$ & \textit{Poseidon is a god from Greek mythology, known} \\
& \textit{as the god of the sea, storms, and earthquakes.} \\ 
& \textit{Neptune is a god from Roman mythology, who is}  \\ 
& \textit{also known as the god of the sea. Both Poseidon and}\\
& \textit{Neptune share similar roles and attributes in} \\
& \textit{their respective mythologies.} \\  
\bottomrule
\end{tabular}}
\caption{An example from StrategyQA dataset, where $X_1$, $R_0$ and $R_1$ are generated by GPT-4.}
\vspace*{-5mm}
\label{tab:example_2}
\end{table}
\paragraph{Reasoning Intervention.} Following \citet{Pearl2001DirectAI}, we conduct counterfactual reasoning to measure the causal effect of a treatment variable on a response variable. We first perform targeted interventions on the input text $X$ and measure their effect on the reasoning outcome $Y$ (direct effect). Further, we also perform interventions on the mediator $R$ and measure their effect on $Y$ (indirect effect). We perform the following steps to automatically generate an intervention on $X$ and $R$. \\  %In a causal graph, the intervening operation on a variable removes all edges pointing to it, so its parent nodes no longer cause it. Figure \ref{fig:causal_graph}(c-d) shows an abstract setting for estimating and removing the direct influence of $X$ on $Y$. 
%Specifically, we perform the following \textit{do}-operation: replace the original input $X_0$ with an alternative input $X_1$. 
\textbf{Step 1: Intervention Data Generation.}  We use a large language model (GPT-4) to automatically generate an alternative treatment variable $X_1$\footnote{See App. \ref{sec:appendix_intervention} for details on task-specific interventions.}. The input to $M$ includes instruction and few-shot examples, taking the format shown in Table \ref{table:counterfactual_prompt}. LLMs can be sensitive to instructions and few-shot examples; hence, we randomize the prompt by manually creating a set of semantically similar instructions. Then, we randomly sample from the instruction set each time. \\
\textbf{Step 2: Manual Data Curation.} To retain high-quality data for our analysis, we manually filter out generated samples from Step 1 that are invalid or low-quality. Table \ref{tab:example_2} shows an example where given the original input reasoning question $X_0$, the model generated $X_1$, where it replaces ``\textit{Vulcan}'' with ``\textit{Neptune}''. To study the direct effect by taking the difference of the model output when we provide them $X_0$, $R_0$ and $X_1$, $R_0$ as inputs.  \\
\textbf{Step 3: Generate Reasoning Chain.} Finally, to get the indirect effect, we generate the reasoning chain ($R_0$, $R_1$) for each reasoning problem $X_0$ or $X_1$ by providing LLMs with some high-level descriptions about each reasoning task and reasoning prompt -- ``\textit{Let’s think step by step}''(see App. \ref{sec:appendix_prompts}). 
%In this work, we measure the faithfulness of LLMs in the setting where the reasoning is sampled before the answer is sampled. Hence, to generate the reasoning chain we provide LLMs with some high-level descriptions about each reasoning task and reasoning prompt -- ``\textit{Let’s think step by step}''. 

%We measure the faithfulness of LLMs in reasoning by observing their behaviour on different intervened input text $X$. 

%In this paper, we focus on studying the effect of the reasoning chain on the final outcomes of the model. Unlike previous \citep{} studies %Hence, we conducted two kinds of studies: (i) for models (>100B) that have the emergent capabilities to generate a plausible chain of reasoning steps and then (ii) 

Our study suggests that vanilla LMs (<20B) (in a zero-shot setting) are systematically unfaithful and consistently fail to reason over the mediator (see Table \ref{tab:open_models_causalresuts}). In general, our experiments show a large variation in the causal effects of COT in the final answer depending on the tasks. Models that are instruction tuned or trained on the chain of thought during the pre-training phase have a better indirect effect across different reasoning tasks, suggesting that fine-tuning on CoT can make the model more faithful (see Table  \ref{tab:closed_models_causal_resuts}). Interestingly, similar to \citet{Turpin2023LanguageMD}, we observe inverse scaling for certain tasks. In our case, the indirect effect worsens with increasingly capable models, indicating that sheer scale might not guarantee faithful reasoning. 


%interventions on the model inputs to reveal the causal role of specific reasoning steps in a model’s behaviour. 

%\textbf{\color{red}{DP: Need to end this section better}}




==> 03_method_copy.tex <==

\section{Method} 

In this section, we propose a new framework \ourmodel{} that focuses on tailoring small-sized LMs (<10B parameters) to be strong rationalizers and perform reasoning faithfully over the rationales. \ourmodel{} aims to improve the synergy between the reasoning chain and the final answer. We will first describe our method to obtain silver reasoning chains from LLMs (GPT-3) ($\S$\ref{sec:inference_module}). Then, we introduce our inference module that trains a model to learn to generate rationales ($\S$\ref{sec:inference_module}). Finally, we will describe our reasoner module, including its training objectives ($\S$\ref{sec:reasoning_module}).

\subsection{Inference Module}\label{sec:inference_module}
In this work, we assume no gold rationales to train our model. Hence, similar to recent works \citep{liu-etal-2022-rainier, liu-etal-2023-crystal, wang-etal-2023-scott, ramnath2024tailoring}, we automatically obtain the silver rationale from LLM (GPT-3) using in-context learning. A common approach is fine-tuning a smaller text-to-text model on the silver rationales generated by LLMs with a standard language modeling loss. Recent studies have shown that fine-tuning models (<5B) on reasoning chains may struggle to \textit{align} the reasoning chains with the provided reasoning question during inference \citep{Yang2023ChainofThoughtIN, pmlr-v202-fu23d}. Additionally, learning to generate a reasoning chain means learning to decompose complex reasoning into smaller reasoning steps implicitly. However, \citet{shridhar-etal-2023-distilling} showed that fine-tuning could lead to learning shortcuts and degrade performance. Recent studies have demonstrated that feedback-based methods can help the model align better with the human goal. Hence, we use Direct Preference Optimization (DPO) \citep{rafailov2023direct} for aligning LMs to learn to generate correct reasoning chains.

\textbf{Preference Data.} We prompt the LLM to generate correct reasoning chains ($R_w$) and incorrect reasoning chains ($R_l$) for each reasoning problem. In our experiments, we consider two kinds of reasoning chains as incorrect: \textit{counterfactual chains} (alternative chains that can lead to different outcomes) and \textit{irrelevant chains}. We assume that models that can understand and learn to prefer correct reasoning chains over counterfactual chains will become more robust and enhance generalization. Hence, we manually construct correct and incorrect intermediate reasoning steps and demonstrate the model with these annotated examples before a new instance is provided. In this way, we obtain a preference data $D \in \{X, R_w, R_l\}$ that contains reasoning problems ($X$) and pairs of reasoning steps that lead to correct ($Y_w$) or incorrect outcomes ($Y_l$).

\textbf{Training.} Given a reasoning problem \{$x \in X$\} and instruction prompt {$p \in$ \{correct or counterfactual}\}, our goal is to train models that could generate reasoning steps ($r_w$ or $r_l$). We propose to adopt Direct Preference Optimization (DPO) \citep{rafailov2023direct}, an effective algorithm for aligning language models with implicit rewards. DPO assumes that we only have access to some pairwise preference data $x \rightarrow$ \{$r_w$ $>$ $r_l$\} for each problem $x \in X$. Hence, while training a model ($\pi_\theta$) to generate correct reasoning steps, we consider counterfactual and irrelevant reasoning steps as less preferred. %Conversely, when training a model ($M_l$) to generate counterfactual reasoning steps, we consider the correct reasoning steps as less preferred. 
Training a DPO model includes two phases: (i) supervised fine-tuning (SFT) and (ii) RL fine-tuning phase.  

\textbf{SFT.} We begin by fine-tuning a pre-trained LM with a maximum log-likelihood objective to obtain $\pi_{sft}$. 

\textbf{RL Phase.} Contrary to traditional RL approaches, which initially train a reward model and subsequently derive a policy from it, DPO enables extracting policy through implicit reward learning. The preference data of human or artificial annotators is modeled by a learnable implicit reward model $f_\theta$ under Bradley-Terry theories \citep{Bradley1952RANKAO}: 

\begin{equation}
     \pi_\theta(r_w > r_l |x) = \sigma(f_\theta(r_w, x) - f_\theta(r_l,x))
\end{equation}
where $\sigma$ is the sigmoid function. To learn $f_\theta$, DPO adopts a binary classification loss: 
\begin{equation}
        L_\text{DPO} = -\mathbb{E}_{\{x,r_w>r_l\}}\text{log}\sigma(f_\theta (r_w,x)  - f_\theta(r_l,x))
\end{equation}

The latent function $f_\theta$ is parameterized by the log-likelihood ratio between $\pi_\theta$ and $\pi_\text{sft}$:
\begin{equation}
    f_\theta(x,r) = \beta\text{log}\frac{\pi_\theta(r|x)}{\pi_\text{sft}(r|x)} 
\end{equation}

where $\beta$ a linear coefficient for scaling $f_\theta$. This parameterization is appealing as it aligns the training of an implicit reward model $f_\theta$ closely with training an LM policy $\pi_\theta$. 

During inference, the reasoning module uses the generated reasoning steps by  $\pi_\theta$ model for a given reasoning problem. 
\begin{figure}[t]
    \centering   
    \includegraphics[scale=1,height=6cm, width=\linewidth]{figure/Frodo.pdf}
    \caption{An overview of \ourmodel{}.}
    \label{fig:main_method}
    \vspace*{-5mm}
\end{figure} 

\subsection{Reasoning Module}\label{sec:reasoning_module} Given a reasoning question $x \in X$ and reasoning steps $r_w$ (correct) and $r_l$ (counterfactual)\footnote{Please note that in the reasoner module, we only consider counterfactual reasoning steps as negative samples.}, our goal is to train a model ($\pi_\gamma$) that can generate a correct answer $y_w$. To encourage our reasoner module to reason faithfully over the reasoning steps, we train the model with a linear combination of two losses: an indirect effect loss and a supervised margin rank loss, $\mathcal{L}= 
\lambda_\text{LM}* \mathcal{L}_{\text{LM}} +  
\lambda_\text{counter}*\mathcal{L}_{\text{counter}} +
\lambda_\text{PREF} *\mathcal{L}_{\text{PREF}} $
, which we describe below.

\textbf{Language Model Loss.} We use the standard training objective to maximize the likelihood of the correct answer using cross-entropy loss, computed as:
\begin{equation}
    \mathcal{L}_{\text{LM}} = -\text{logP}(y_w|x,r_w)
\end{equation}

\textbf{Counterfactual Loss.} To encourage the model to reason robustly and faithfully towards the reasoning steps, we propose training the model to learn how different reasoning chains (correct or counterfactual) can lead to different outcomes. Hence, inspired by the causal mediation theory \citep{Pearl2001DirectAI}, we use the following loss: 
\begin{equation}
     \mathcal{L}_{\text{counter}} = - {\text{logP}(y_l|x,r_l)}
\end{equation}

Similar to \citep{wang-etal-2023-scott, Roese1997CounterfactualT}, we posit that adding a counterfactual objective can help the model to avoid learning reasoning shortcut between a question and the gold answer since now the model is tasked to answer differently for the same question.

\textbf{Margin-Ranking Loss.} It has been shown \citep{khosla2020supervised} that contrastive loss and ranking loss help to improve model robustness and generalization against input variation. Hence, we propose to use the margin ranking loss that aims to maximize the margin between positive examples (i.e., statements containing questions, correct reasoning steps and correct answers) and negative examples (i.e., statements containing questions, counterfactual reasoning steps and correct answers). 

% \begin{equation}
%      \mathcal{L}_{\text{PREF}}= max(0, t*\underbrace{(logP(x,r_w,y_w) -
%      logP(x,r_l,y_w))}_{\text{indirect effect}} \\
%      +{m})
% \end{equation}

\begin{equation}
     \mathcal{L}_{\text{PREF}}= max(0, t*\text{IE}+{m})
\end{equation}

where $t$ is the label (indicating which sample in the pair is better), $m$ is the margin, and the indirect effect IE = $h(x,r_w,y_w) - h(x,r_l,y_w)$ where $h$ is the logits. 



%Counterfactual reasoning  \citep{} is a statistical inference method used to infer outcomes under hypothetical conditions that are different from the factual world. 








==> 05_results_copy.tex <==











\section{Results}

%One intuitive reason could be that instruction tuning helps the model learn an effective way to align the output to its input \citep{liu2024what}. In contrast, RLHF techniques are trained to optimize rewards derived from human feedback based on the quality of the generation rather than on faithfulness in reasoning \citep{sharma2024towards}. 

\begin{table}[t!]
\centering
\footnotesize
\scalebox{0.9}{
\begin{tabular}{lcccc}
\toprule 
  \textbf{Models}
 & \textbf{StrategyQA}
 & \textbf{QuaRel}
 & \textbf{OBQA} 
 & \textbf{QASC}  \\
 \midrule
\textbf{GPT-$3.5^{\diamond}$}  &  69.7  & 83.4 & 84.5 &  80.3 \\ 
\midrule
\textbf{SFT}  &   \cellcolor{teal!25}57.6 &  \cellcolor{teal!25}74.6   & \cellcolor{teal!25}65.0 &   \cellcolor{teal!25}58.6 \\ 
\textbf{SFT + CoT}  &  \cellcolor{teal!25}63.6 & \cellcolor{teal!25}77.7 & \cellcolor{teal!25}65.5 & \cellcolor{teal!25}59.4 \\ 
\textbf{Rainier}  & \cellcolor{teal!25} --   &  \cellcolor{teal!25}-- &  \cellcolor{teal!25}69.7 & \cellcolor{teal!25}54.9 \\ 
\textbf{Crystal}  &   \cellcolor{teal!25}-- &  \cellcolor{teal!25}-- &  \cellcolor{teal!25}64.2 & \cellcolor{teal!25}56.8 \\ 
\textbf{\textsc{Mario}}  &   \cellcolor{teal!25}65.1  &  \cellcolor{teal!25}79.9 & \cellcolor{teal!25}66.1  & \cellcolor{teal!25}60.1 \\ 
\textbf{\ourmodel{}}  &  \cellcolor{teal!25}\textbf{68.4}$^*$  &  \cellcolor{teal!25}\textbf{83.4}$^*$ & \cellcolor{teal!25}70.2$^+$  & \cellcolor{teal!25}\textbf{64.2}$^*$\\ 
\textbf{-DPO} &  \cellcolor{teal!25}{66.2}  &  \cellcolor{teal!25}{82.2} &  \cellcolor{teal!25}68.1 & \cellcolor{teal!25}{62.4} \\
\textbf{-CL} &  \cellcolor{teal!25}{65.2}  &  \cellcolor{teal!25}{82.1} & \cellcolor{teal!25}66.4  & \cellcolor{teal!25}{60.1} \\ 
\textbf{-MRL} &  \cellcolor{teal!25}{65.5}  &  \cellcolor{teal!25}{81.3} &\cellcolor{teal!25} 66.2  & \cellcolor{teal!25}{62.1}\\ 
\midrule
\textbf{SFT}  &  \cellcolor{pink!25}63.1 & \cellcolor{pink!25}81.29 &	\cellcolor{pink!25}72.0 &	\cellcolor{pink!25}67.8 \\ 
\textbf{SFT + CoT}  & \cellcolor{pink!25}65.1	& \cellcolor{pink!25}84.2	& \cellcolor{pink!25}73.3	& \cellcolor{pink!25}72.0 \\ 
\textbf{SCOTT} & \cellcolor{pink!25}{61.5}&\cellcolor{pink!25} --& \cellcolor{pink!25}-- & \cellcolor{pink!25}{65.0} \\
\textbf{Crystal}  &  \cellcolor{pink!25}-- &  \cellcolor{pink!25}-- &  \cellcolor{pink!25}78.3 & \cellcolor{pink!25}74.3 \\ 

\textbf{\ourmodel{}}  & \cellcolor{pink!25}\textbf{82.1}$^*$ & \cellcolor{pink!25}\textbf{93.5}$^*$ &  \cellcolor{pink!25}\textbf{80.1}$^*$  &  \cellcolor{pink!25}\textbf{75.9}$^*$ \\
\midrule
\textbf{LlaMa-2-7B}  & \cellcolor{yellow!25}67.2  \\ 
\textbf{SFT + CoT}  & \cellcolor{yellow!25}79.4 \\
\textbf{\ourmodel{}} & \cellcolor{yellow!25} 81.5 \\
\midrule
\textbf{Mistral-7B}  &  \cellcolor{cyan!25}58.2  \\ 
\textbf{SFT + CoT}  & \cellcolor{cyan!25}80.2 \\
\textbf{\ourmodel{}} & \cellcolor{cyan!25}81.9 \\
\bottomrule
\end{tabular}}
\caption{Performance of small-sized LMs (770M-7B) on four different reasoning tasks. The base models are \colorbox{teal!25} {T5-large} (770M),  \colorbox{pink!25}{T5-3B} (3B), \colorbox{yellow!25}{LLaMa-2-7B} and \colorbox{cyan!25}{LLaMa-2-7B} . We report accuracy (\%).{$^\diamond$}: few-shot performance, $^*$: p-value<0.01, $^+$: p-value<0.05 }\label{tab:main_resuts}
\vspace*{-5mm}
\end{table}
\textbf{Comparing \ourmodel{} with baselines.} We now empirically compare \ourmodel{} with three strong baseline models (see Table \ref{tab:main_resuts}). We consider T5-large (770M) as the inference and reasoning modules. We have the following three observations. First, we present the performance of GPT-$3.5$ on these tasks. We observe the performance on StrategyQA is much lower than on other tasks, indicating the rationales generated for this task can be unfaithful. Hence, similar to \citep{ramnath2024tailoring}, for training \ourmodel{}, we use only the instances where the answer predicted by GPT-$3.5$ is correct. Second, for all four datasets, we observe that \ourmodel{} outperforms the strong self-rationalization baselines. \ourmodel{}, on average, improves the performance by +$4.1$ and +$3$ accuracy points compared to the SFT + CoT and \textsc{Mario} (the strongest baseline), respectively, across all four tasks. Since SFT + CoT and \textsc{Mario} use the same knowledge from GPT-3.5, our results suggest that both our inference and reasoning modules bring substantial performance gains to the model. Third, it is worth noting that increasing (large to 3B) the model size does not hamper the performance of \ourmodel{}. 

%Table 3 shows the comparisons between MARIO and the baselines. For all five datasets, we note that MARIO is the overall best setup as noted by both the individual metrics and the averaged NRG metric. ADDITIVE MARIO is found to be the best performing method for STRATEGYQA, and CANONICAL MARIO is found to be the best method for the other 4 datasets. It is important to note that not only does the rationale get better, but the task accuracy also shows a marked improvement over the baselines. We show some representative examples of rationales generated by training with MARIO, in comparison with those generated by SFT in Table 4. We also release the rationales generated by SFT and MARIO.

\textbf{Ablation.} To obtain a better insight into the contribution of each component of \ourmodel{}, we perform an ablation study (see Table. \ref{tab:main_resuts}). First, when we do not use the DPO to train our inference module, we see a consistent drop (-$1.9\%$) in performance across the four tasks, indicating the importance of incorporating implicit feedback provided by the DPO in the model's training. Further, we observe a considerable drop in performance when we do not use counterfactual (-$3.1\%$) and margin ranking loss (-$2.8\%$). This result highlights the model's ability to benefit from including counterfactual examples. \\
\vspace*{-5mm}






















%Conversely, XXXX models 

%Even though larger models assign a higher probability to the correct more often, this does not necessarily translate to a larger margin between the probability of the correct and incorrect options.

==> dump.tex <==

\begin{table*}[t!]
\centering
%\footnotesize
\scalebox{0.7}{
\begin{tabular}{lccccccc}%ccccccccccc}
\hline 
   \multirow{2}{}{\textbf{Models}}
 & \multicolumn{7}{c}{{\textbf{StrategyQA}}} 
 %& \multicolumn{4}{c}{{\textbf{GSM8K}}}
 %& \multicolumn{4}{c}{{\textbf{FOLIO}}}
   \\
{} & \multicolumn{1}{c}{w/o CoT} & \multicolumn{1}{c}{CoT}& \multicolumn{1}{c}{Oracle Knowledge}& \multicolumn{1}{c}{Counterfactual Knowledge} & \multicolumn{1}{c}{Oracle CoT} & \multicolumn{1}{c}{Counterfactual CoT} & \multicolumn{1}{c}{Confounder CoT} \\  \hline 
 %\multicolumn{1}{c}{w/o CoT} & \multicolumn{1}{c}{CoT} & \multicolumn{1}{c}{Oracle}& \multicolumn{1}{c}{Counterfactual}& 
 %\multicolumn{1}{c}{w/o CoT} & \multicolumn{1}{c}{CoT}& \multicolumn{1}{c}{Oracle}&  \\ 

\textbf{LLaMa-2-7B}  & 62.0  &  {} &  59.6 &  47 & 70.2 & 48.8 & 66  \\%& 22.3 & 41.2 & 21.3 \\%& 0.0 & 0.0 & 0.0 & 0.0  \\ 

%\textbf{T0-11B}        & 57.6  & -- & 81.0 & 40.6 & \\ %& 0.0 & 0.0 & 8.94 & 0.0 & 0.0 & 0.0 & 0.0 \\
\textbf{Stable-Vicuna-13B}  & 38.4  & {--} & 81.0 & 40.6 & 0.0 & 0.0 & 39.8\\ %& 0.0 & 0.0 & 8.94 & 0.0 & 0.0 & 0.0 & 0.0  \\
%\textbf{Flan-T5-11B$^\heartsuit$}    & 66.0  & 67.6 &  92.2 & 53.5 & 92.2 & 68.4\\%& 9.9 \\%& 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\ \vspace*{0.2cm} 
\textbf{LLaMa-33B} &  51.6 &  {--} &  64 & 41.8  & 57.8 & 50.1 & 41 \\
\textbf{GPT-3}  & 54.4  & 58.8 & 75.2 $\pm 3.3 $ & 58.2 $\pm$ 3.2 & 86  & 65.3 & 73.8 \\  %& 18.6 & 56.4 &  73.8 & 50.1 \\%&  0.0 & 0.0 & 0.0  \\ 
 
\textbf{GPT-4$^\clubsuit$}  & 73.4 & 78.4 & 92.2 & 59.6 $\pm$ 2.4  & 94  & 51.1 & 83.2 \\ 
\hline 
\end{tabular}}
\caption{Zero-Shot Setting: Performance of LLMs on Reasoning over a Chain. Accuracy (\%) }\label{tab:main_resuts}
\end{table*}





\if false
\begin{table}[t!]
\centering
\footnotesize
\scalebox{0.9}{
\begin{tabular}{llrrr}
\hline 
   {\textbf{Models}}
 & {{\textbf{StrategyQA}}} 
 & {{\textbf{GSM8K}}}
 & {{\textbf{Logical}}} \\
\hline \\
\textbf{LLaMa-2-13B} & & 28.7\\ 
\textbf{GPT-3} & &19.8&\\
\textbf{GPT-4} & & 51.8 &\\
\hline
\end{tabular}}
\caption{Inertia of LLMs $\delta$ score }\label{tab:main_resuts}
\end{table}


\begin{table}[t!]
\centering
\footnotesize
\scalebox{0.9}{
\begin{tabular}{lrrr}
\hline 
   {\textbf{Models}}
 & {{\textbf{StrategyQA}}} 
 & {{\textbf{GSM8K}}}
 & {{\textbf{Logical}}} \\

\textbf{LLaMa-2-13B} & & 28.7\\ 
\textbf{GPT-3} & &19.8&\\
\textbf{GPT-4} & & 51.8 &\\
\hline
\end{tabular}}
\caption{Error of LLMs}\label{tab:main_resuts}
\end{table}

\fi 

\begin{table}
\parbox{.4\linewidth}{
\begin{tabular}{lrrr}
\hline 
   {\textbf{Models}}
 & {{\textbf{StrategyQA}}} 
 & {{\textbf{GSM8K}}}
 & {{\textbf{Logical}}} \\
\hline \\
\textbf{LLaMa-2-13B} & & 29.1& \\ 
\textbf{GPT-3} & &19.8&\\
\textbf{GPT-4} & & 51.8 &\\
\hline
\end{tabular}}
\caption{Inertia of LLMs}
\hfill
\parbox{.4\linewidth}{
\centering
\begin{tabular}{lrrr}
\hline 
   {\textbf{Models}}
 & {{\textbf{StrategyQA}}} 
 & {{\textbf{GSM8K}}}
 & {{\textbf{Logical}}} \\
\hline \\
\textbf{LLaMa-2-13B} & & 45 &\\ 
\textbf{GPT-3} & &33&\\
\textbf{GPT-4} & & 12.4 &\\
\hline
\end{tabular}
\caption{Error of LLMs}}
\end{table}


\begin{table}[t!]
\centering
\footnotesize
{
\begin{tabular}{lccc}
\hline  
   {\textbf{Models}}
 & {{\textbf{StrategyQA}}} 
 & {{\textbf{GSM8K}}}
 & {{\textbf{FOLIO}}} \\

\hline 
%\textbf{LLaMa-2} & & 41.2 \\
%\textbf{LLaMa-2 + FR} & & 81.4 \\ 
%\textbf{GPT-3} & & &\\
%\textbf{GPT-4 + FR} & & &\\
%\textbf{GPT-4} & & &\\
%\textbf{GPT-4 + FR} & & &\\
w/o Reasoning Chain & 67.86 & 0.0 &0 \\
w/o Reasoning Chain + Logic (During Training) & 69.46 & 0.0 &0 \\
w/o Reasoning Chain + Logic (MTL) & 67.66 & 0.0 & 0 \\
w/o Reasoning Chain + Logic (Symbolic Loss) & 69.08 & 0.0 & 0 \\
w/o Reasoning Chain + Logic (PPO) & .0 & 0.0 &0 \\

RC$_{GPT-4}$ + R$_{Finetune}$ & 74.05/53.9 & 0.0 &0 \\ 

RC$_{GPT-4}$ + Logic Adapter+ R$_{Finetune}$ & 76.04/0.0 & 0.0 &0 \\
RC$_{Oracle}$ + R$_{Finetune}$ & 85.4/57.5 & 0.0 &0 \\ 


\hline 
\end{tabular}}
\caption{Methods to Improve the performance. Model: Flan-T5-large  }\label{tab:main_resuts}
\end{table}


\begin{table*}[t!]
\centering
\footnotesize
\scalebox{0.6}{
\begin{tabular}{lccccccccccccccccccccccc}
\toprule 
   \textbf{Models}
 & \multicolumn{6}{c}{{\textbf{StrategyQA}}} 
 & \multicolumn{6}{c}{{\textbf{GSM8k}}}
 & \multicolumn{6}{c}{{\textbf{Causal Understanding}}}
   \\
 & \multicolumn{1}{c}{Vanilla} & \multicolumn{1}{c}{RC} & \multicolumn{2}{c}{CIE} & \multicolumn{2}{c}{CDE} 
 & \multicolumn{1}{c}{Vanilla} & \multicolumn{1}{c}{RC} & \multicolumn{2}{c}{CIE} & \multicolumn{2}{c}{CDE} 
  & \multicolumn{1}{c}{Vanilla} & \multicolumn{1}{c}{RC} & \multicolumn{2}{c}{CIE} & \multicolumn{2}{c}{CDE} \\ 
\midrule
\textbf{Flan-Alpaca-3B} & 62.2 &  & \cellcolor{pink!25}0.15 & \cellcolor{blue!25} -0.28 &  \cellcolor{pink!25} 0.52 & \cellcolor{blue!25} -0.26 & 2.8 &  20.3 & \cellcolor{pink!25} 0.60 & \cellcolor{blue!25} 0.53 & \cellcolor{pink!25} 0.35 & \cellcolor{blue!25} 0.70 &  59.4 & 61.7 & \cellcolor{pink!25} 0.03 &	\cellcolor{blue!25} 0.28 &	\cellcolor{pink!25} 0.01 & \cellcolor{blue!25} -0.02\\  

\textbf{LLaMa-2-7B}  & 57.5 & 71.3 & \cellcolor{pink!25}0.44 & \cellcolor{blue!25} 0.20 &\cellcolor{pink!25} 0.36 & \cellcolor{blue!25} 0.05 & 10.9 & 61.1 & \cellcolor{pink!25} 0.55 & \cellcolor{blue!25} -0.04 & \cellcolor{pink!25} -0.03 & \cellcolor{blue!25} -0.01 & 46.2 & 53.7 & \cellcolor{pink!25} 0.03 & \cellcolor{blue!25} -0.02 & \cellcolor{pink!25}0.03	& \cellcolor{blue!25} -0.18 \\ 

\textbf{Mistral-7B} & 59.2 & 82.2 &  \cellcolor{pink!25} 0.34 & \cellcolor{blue!25} 0.34  & \cellcolor{pink!25} 0.61 & \cellcolor{blue!25} 0.16  & 10.9 &  70.1 & \cellcolor{pink!25} 0.59  & \cellcolor{blue!25} 0.01 & \cellcolor{pink!25} -0.01 & \cellcolor{blue!25} -0.01 & 44.5 & 44.5 & 
\cellcolor{pink!25} 0.24 & \cellcolor{blue!25}0.41 &	\cellcolor{pink!25}-0.04 &	\cellcolor{blue!25}0.14  \\ 


\textbf{Flan-T5-11B} & 64.4 & 85.6 & \cellcolor{pink!25} 0.35 & \cellcolor{blue!25} 0.08 & \cellcolor{pink!25} 0.65 & \cellcolor{blue!25} -0.57 & 3.7 & 39.3 & \cellcolor{pink!25} 0.79& \cellcolor{blue!25} 0.54 & \cellcolor{pink!25} 0.25 & \cellcolor{blue!25} -0.06 & 60.5 & 62.5 & \cellcolor{pink!25} 0.13 &	\cellcolor{blue!25}0.16& \cellcolor{pink!25}	-0.22	& \cellcolor{blue!25}0.13\\ 


\textbf{LLaMa-2-13B} & 50.0 & 80.0 & \cellcolor{pink!25} 0.49 &  \cellcolor{blue!25} 0.44 & \cellcolor{pink!25} 0.58 & \cellcolor{blue!25} 0.14  & 9.0 & 65.4 & \cellcolor{pink!25} 0.58 & \cellcolor{blue!25} -0.01 &  \cellcolor{pink!25} 0 & 
\cellcolor{blue!25} -0.01 & 52.5 & 54.2 &  \cellcolor{pink!25} 0.15 & \cellcolor{blue!25}	-0.02 &	 \cellcolor{pink!25} 0.04	& \cellcolor{blue!25}-0.01 \\ 

\midrule
\textbf{LLaMa-2-70B} & 43.2 & 53.3 &  \cellcolor{pink!25} 0.056 & 
 -- & \cellcolor{pink!25} 0.09 & -- & 14 & 68.2 & \cellcolor{pink!25} 78.0 & -- & \cellcolor{pink!25} 82.0 & -- & 50.8 & 57.5 & \cellcolor{pink!25}0.07 & -- & \cellcolor{pink!25}0.13 & --\\
\bottomrule
\end{tabular}}
\caption{\textbf{Causal Effects} with the controlled reasoning chains.}\label{tab:appnopen_models_causalresuts}
\end{table*}








\begin{table*}[t!]
\centering
\footnotesize
\scalebox{0.9}{
\begin{tabular}{lccccccccccccccccc}
\toprule 
   \textbf{Models}
 & \multicolumn{4}{c}{{\textbf{StrategyQA}}} 
 & \multicolumn{4}{c}{{\textbf{GSM8k}}}
 & \multicolumn{4}{c}{{\textbf{Causal Understanding}}}
   \\
 & \multicolumn{2}{c}{CIE} & \multicolumn{2}{c}{CDE} 
 & \multicolumn{2}{c}{CIE} & \multicolumn{2}{c}{CDE} 
 & \multicolumn{2}{c}{CIE} & \multicolumn{2}{c}{CDE} \\ 
\midrule
\textbf{Flan-Alpaca-3B} & \cellcolor{pink!25}0.15 & \cellcolor{blue!25} -0.28 &  \cellcolor{pink!25} 0.52 & \cellcolor{blue!25} -0.26 &  \cellcolor{pink!25} 0.60 & \cellcolor{blue!25} -0.01 & \cellcolor{pink!25} 0.35 & \cellcolor{blue!25} 0.06 & \cellcolor{pink!25} -0.01 &	\cellcolor{blue!25} 0.28 &	\cellcolor{pink!25} 0.01 & \cellcolor{blue!25} -0.02\\  

\textbf{LLaMa-2-7B}  & \cellcolor{pink!25}0.44 & \cellcolor{blue!25} 0.20 &\cellcolor{pink!25} 0.36 & \cellcolor{blue!25} 0.05 & \cellcolor{pink!25} 0.55 & \cellcolor{blue!25} -0.04 & \cellcolor{pink!25} -0.03 & \cellcolor{blue!25} -0.01 &  \cellcolor{pink!25} 0.03 & \cellcolor{blue!25} -0.02 & \cellcolor{pink!25}0.03	& \cellcolor{blue!25} -0.18 \\ 

\textbf{Mistral-7B} & \cellcolor{pink!25} 0.34 & \cellcolor{blue!25} 0.34  & \cellcolor{pink!25} 0.61 & \cellcolor{blue!25} 0.16 & \cellcolor{pink!25} 0.59  & \cellcolor{blue!25} 0.01 & \cellcolor{pink!25} -0.01	& \cellcolor{blue!25} -0.01 &  
\cellcolor{pink!25} 0.24 & \cellcolor{blue!25}0.41 &	\cellcolor{pink!25}-0.04 &	\cellcolor{blue!25}0.14  \\ 


\textbf{Flan-T5-11B} & \cellcolor{pink!25} 0.35 & \cellcolor{blue!25} 0.08 & \cellcolor{pink!25} 0.65 & \cellcolor{blue!25} -0.57 
& \cellcolor{pink!25} 0.79& \cellcolor{blue!25} 0.54 & \cellcolor{pink!25} 0.25 & \cellcolor{blue!25} -0.06 & 
\cellcolor{pink!25} 0.13 &	\cellcolor{blue!25}0.16 & \cellcolor{pink!25}	-0.22	& \cellcolor{blue!25}0.13\\ 


\textbf{LLaMa-2-13B} & \cellcolor{pink!25} 0.49 &  \cellcolor{blue!25} 0.44 & \cellcolor{pink!25} 0.58 & \cellcolor{blue!25} 0.14  &
\cellcolor{pink!25} 0.58 & \cellcolor{blue!25} -0.01 &  \cellcolor{pink!25} 0 & \cellcolor{blue!25} -0.01 & 
\cellcolor{pink!25} 0.15 & \cellcolor{blue!25}	-0.02 &	 \cellcolor{pink!25} 0.04 & \cellcolor{blue!25}-0.01 \\ 

\midrule
\textbf{LLaMa-2-70B} & \cellcolor{pink!25} 0.05 & 
 -- & \cellcolor{pink!25} 0.09 & -- & \cellcolor{pink!25} 0.78 & -- & \cellcolor{pink!25} 0.82 & -- & \cellcolor{pink!25}0.07 & -- & \cellcolor{pink!25}0.13 & --\\
\bottomrule
\end{tabular}}
\caption{\textbf{Causal Effects} with the controlled reasoning chains.}\label{tab:appendix_open_models_causalresuts}
\end{table*}





==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

